Perspectives on few-body cluster structures in exotic nuclei

It is a fascinating phenomenon in nuclear physics that states with a pronounced few-body structure can emerge from the complex dynamics of many nucleons. Such halo or cluster states often appear near the boundaries of nuclear stability. As such, they are an important part of the experimental program beginning at the Facility for Rare Isotope Beams (FRIB). A concerted effort of theory and experiment is necessary both to analyze experiments involving effective few-body states, as well as to constrain and refine theories of the nuclear force in light of new data from these experiments. As a contribution to exactly this effort, this paper compiles a collection of ``perspectives'' that emerged out of the Topical Program ``Few-body cluster structures in exotic nuclei and their role in FRIB experiments'' that was held at FRIB in August 2022 and brought together theorists and experimentalists working on this topic.

==> stash.tex <==
% MOVED FROM SECTION 3

\begin{itemize}
%   \item Motivation: experimental interest, unnuclei, interest in many-neutron halos
%    \item Introduction: low-energy universal dynamics (general perspective, short-range interactions, EFT)
    \item Overview of available technology that can do high-precision calculations: Faddeev for three-body, CGHS for 4,5, maybe more
    \begin{itemize}
        \item Capabilities and trade-offs for different methods
        \item Potential improvements in future work
        \item Mutual benchmarking
        \item Need to handle optical potentials
    \end{itemize}
    
    \item For the paragraph or two on hyperspherical methods (Higgins)
    \begin{itemize}
        \item Give an overview of applications of the hyperspherical approach (i.e. for both using hyperspherical harmonics as a basis, and using the adiabatic hyperspherical approach) in atomic and nuclear systems.
        \item Maybe discuss the applications of the ECG basis in nuclear problems.
        \item List benefits of this approach and what can be done with this approach that others might not.
        \item Give an outlook on possible nuclear processes that would be possible to study in the hyperspherical method.
    \end{itemize}
%    \item Observables to be calculated, possible future experiments (d,p), (d,n)
%    \item What do we learn from all this?  E.g., evolution of universality along isotopic chains.
\end{itemize}

\subsection{Discussion/Brainstorming August 17}

\begin{itemize}
\item Try to find islands of model independence (few-body universality) to be probed with transfer reactions
   \begin{itemize}
   
    \item Weak model dependence: once potential is fitted to key low-energy observables from two-body experimental data or realistic model calculations
    
    \item Prediction of halo properties independent of details of interaction
    
    \item Look for small one, two or several neutron separation energies (Emiko HIYAMA $^8$He five-body problem)

   \end{itemize}

\item Check for universality in reactions along the dripline

   \begin{itemize}
    \item Use $(d,p)$ reactions to study halos, $(d,np)$ with $E_{np}\approx0$ (quasi-free kinematics) to study halos in the continuum, e.g., $^9$Li($d$ , $p$)$^9$Li-$n$
    
    \item Use $(t,p)$ reactions to study 2-neutron halos with $S_{2n}\approx 0$  
   \end{itemize}

\item Single theory implementation can simultaneously give answers for different systems
\begin{itemize}
 \item Existing Faddeev framework (Hlophe et al.) can handle (d,n) and (d,p) reactions in full three-body framework
 \item For nucleon-core interactions, optical potentials are needed
 \item If systems are universal, it should be possible to use simple models for neutron-core interactions
 \item Opportunity to study virtual states
  \begin{itemize}
   \item Experimental signature is enhancement in cross sections
   \item Theory can look for virtual-state pole directly in complex plane
  \end{itemize}
\end{itemize}
\item Comprehensive calculation describes reaction mechanism and final-state interaction at the same time
 \begin{itemize}
  \item Discuss what can be done within three-body formalism: limitations of Faddeev approach
  \item Provide a roadmap/perspective for complete four-body calculations
  \item Faddeev-Yakubowsky is an obvious possibility
  \item But hyperspherical formalism with correlated Gaussians (Higgins et al.) can also handle reaction calculations (3--5, possibly 6--body systems-but computationally challenging/expensive for systems larger than 4 or 5)
   \begin{itemize}
    \item The adiabatic hyperspherical method has been extensively used in studying cold and ultra--cold atomic collisions: computing three--body recombination (i.e. $A+A+B\rightarrow A+AB$ [], ect.), some four--body recombination rates (i.e. the formation of Efimov trimers in the recombination process $B+B+B+B\rightarrow B_3+B$ []). 
    \item Existing formalism can accommodate systems of a core plus a few neutrons, with examples such as $^{10}\mathrm{Be}+n+n$ and $^{4}\mathrm{He}+n+n$.
    \item Currently, all potentials have to be real, should be possible to include imaginary part
    \item At low energies, imaginary parts should be small: benchmark with real calculations
    \item The adiabatic hyperspherical treatment can treat central, spin--orbit, and tensor two--body interactions, as well as three--body forces.
    \item Unclear how to utilise the adiabatic hyperspherical treatment for non--local interactions but can use local $l$--dependent potentials, like in the case of the $^{10}\mathrm{Be}+n+n$ system to study states of $^{12}\mathrm{Be}$ [PRC 77, 054313 (2008) and PRC 86, 024310 (2012)].
    \item One could study knockout reactions such as the four-body system of $\alpha+n+n+p$ to look at $^{6}\mathrm{He}(p,p\alpha)nn$, or more computationally rigorous six--body reactions $^8\mathrm{He}(p,p\alpha)4n$, and $^{4}\mathrm{He}(^{8}\mathrm{He},^{8}\mathrm{Be})4n$ (model $^{8}\mathrm{Be}$ as a composite nucleus of two $\alpha$ cores).
   \end{itemize}
   
  \item Generally, identify list of groups who can work on such calculations
 \end{itemize}
\end{itemize}
